Beyond Interval MDPs: Tight and Efficient Abstractions of Stochastic Systems

This work addresses the general problem of control synthesis for continuous-space, discrete-time stochastic systems with probabilistic guarantees via finite abstractions. While established methods exist, they often trade off accuracy for tractability. We propose a unified abstraction framework that improves both the tightness of probabilistic guarantees and computational efficiency. First, we introduce multi-interval MDPs (MI-MDPs), a generalization of interval-valued MDPs (IMDPs), which allows multiple, possibly overlapping clusters of successor states. This results in tighter abstractions but with increased computational complexity. To mitigate this, we further propose a generalized form of MDPs with set-valued transition probabilities (SMDPs), which model transitions as a fixed probability to a state cluster, followed by a non-deterministic choice within the cluster, as a sound abstraction. We show that control synthesis for MI-MDPs reduces to robust dynamic programming via linear optimization, while SMDPs admit even more efficient synthesis algorithms that avoid linear programming altogether. Theoretically, we prove that, given the partitioning of the state and disturbance spaces, both MI-MDPs and SMDPs yield tighter probabilistic guarantees than IMDPs, and that SMDPs are tighter than MI-MDPs. Extensive experiments across several benchmarks validate our theoretical results and demonstrate that SMDPs achieve favorable trade-offs among tightness, memory usage, and computation time.

==> sections_old/approach_old.tex <==
\section{UMDP Abstraction}
\label{sec:abstraction}

We present two methods of constructing sound UMDP abstractions that admit high quality controller synthesis results for System~\eqref{eq:sys} given $\varphi$-respecting partition $S$. Both methods rely on reachable set computations for each region $s \in S$ under nonlinear dynamics $f$.
% 
% Since we assume a general nonlinear $f$, our abstractions rely on reachable set computations.
%
\begin{definition}[$\mathrm{Reach}$]
    The $1$-step forward reachable set of $s\subset \reals^n$, $u \in U$, and $c \in W$ is defined as $\mathrm{Reach}(s,a,c) := \{f(x,a,w) : x\in s, w \in c\}$.
\end{definition}
%
There exist numerous approaches to obtain (overapproximations) of $\mathrm{Reach}$, e.g., \ig{(CITE)}.
% \ml{it's unclear how to handle the case when $P_w$ is unknown.}
% We note that, for our framework, it is sufficient to have an over-approximation of $\mathrm{Reach}$, i.e., it does not compromise the soundness of our framework but increases its conservatism.
In our framework, an overapproximation of $\mathrm{Reach}$ is sufficient, i.e., it does not affect soundness but may increase conservatism.
% 
% \subsection{States, Actions and Disturbance Partition}
% 
% Furthermore, both We also partition the set $W$ of System~\eqref{eq:sys}, obtaining $C$.
%
Furthermore, both of our UMDP abstraction classes also use a partition $C := \{c_i, \dots, c_{|C|} \}$ of the disturbance set $W$.

\subsection{UMDP-Poly Abstraction}
Our first method of abstraction constructs ambiguity set $\Gamma^\poly$ in the form of a polytope.  This method generalizes IMDP abstraction \cite{lahijanian2015formal, givan2000bounded}, where $\Gamma$ is rectangular, as well as the 2-layer UMDP abstraction in \cite{gracia2024temporal}, which also obtains a polytopic $\Gamma$. Contrary to IMDPs, we define $\Gamma^\poly_{s,a}$ by setting bounds on the probability that the successor state of $(s,a)$ belongs to a set (or cluster) of states of $\U^\poly$, rather than a single successor. Specifically, these clusters might in principle be overlapping, thus generalizing the approach of \cite{gracia2024temporal}. In order to define $\Gamma^\poly$, we first state the following technical lemma.

%
\begin{lemma}
    \label{lemma:tp_bounds}
    Consider a region $s\in S_\safe$, action $a\in A$, and the partition $C$ of the disturbance space $W$, and let $\tilde s \subseteq \reals^n$. The probability of transitioning from each $x\in s$ to the region $\tilde s$ under action $a\in A$ satisfies
    %Let $\tilde s := \cup_{i = 1}^m s_i$ be an arbitrary union (cluster) of regions $s_1, \dots, s_m \in S$. Consider the state region $s\in S_\safe$, disturbance region $c \in C$, and action $a\in A$. %The probability of transitioning from each $x\in s$ to the cluster $\tilde s$ under action $a\in A$ satisfies 
    $\kernel(\tilde s \mid x, a) \in [\underline P(s, a, \tilde s), \overline P(s, a, \tilde s)]$, where
    %
    \begin{subequations}
        \label{eq:tp_bounds}
        \begin{align}
            \underline P(s, a, \tilde s) &:= \sum_{c \in C} \boldsymbol{1}(\mathrm{Reach}(s,a,c) \subseteq \tilde s)P_w(c),
            \label{eq:tp_bounds_lower}\\
            \overline P(s, a,\tilde s) &:= \sum_{c \in C} \boldsymbol{1}(\mathrm{Reach}(s,a,c) \cap \tilde s \neq \emptyset)P_w(c).
             \label{eq:tp_bounds_upper}
        \end{align}
    \end{subequations}
 %
\end{lemma}
\begin{proof}
    Start by considering the lower bound. By \cite[Proposition 4.1]{gracia2024temporal}, it holds that
    %
    %\begin{align*}
        $\kernel(\tilde s \mid x, a) \ge P(\{w\in W: \mathrm{Reach}(s,a,w) \subseteq \tilde s\}) = \sum_{c\in C} P(\{w\in c: \mathrm{Reach}(s,a,w) \subseteq \tilde s\})$,
    %\end{align*}
    %
    where the equality follows from the law of total probability by noting that $C$ is a partition of $W$. Then, since for each $c\in C$, we have that $\mathrm{Reach}(s,a,c) \subseteq \tilde s \implies \mathrm{Reach}(s,a,w) \subseteq \tilde s$ for all $w\in c$, we obtain $\{w\in c: \mathrm{Reach}(s,a,w) \subseteq \tilde s\} \supseteq \{w\in c: \mathrm{Reach}(s,a,c) \subseteq \tilde s\}$, which is equal to $c$ if $\mathrm{Reach}(s,a,c) \subseteq \tilde s$, otherwise being the empty set. Therefore, it follows that $P(\{w\in c: \mathrm{Reach}(s,a,w) \subseteq \tilde s\})\ge \boldsymbol{1}( \mathrm{Reach}(s,a,c) \subseteq \tilde s ) P(c)$ for all $c\in C$, yielding the desired lower bound. The upper bound follows from the same logic.
\end{proof}

\begin{remark}
    In the case that $P$ is unknown and samples $\{\w^i\}$ from it are available, similar bounds to \eqref{eq:tp_bounds} are given in \cite{gracia2024temporal}, which involve the reachable sets $\{\mathrm{Reach}(s,a,\w^i)\}$, and which hold with a confidence.
\end{remark}

We now formally define our UMDP-Poly abstraction and prove its soundness:
%
\begin{definition}[UMDP-Poly Abstraction]
    \label{def:mdp_poly_abstraction}
    Let $\widetilde S\subseteq 2^S$ be a set of (possibly overlapping) unions (clusters) of regions (states) in $S$, i.e., each $\tilde s \in \widetilde S$ can be written as $\tilde s := \cup_{i = 1}^m s_i$, for some $s_1, \dots, s_m \in S$. For each state-action pair $s\in S_\safe, a \in A$, let $\widetilde S_{s,a}$ denote an arbitrary subset of $\widetilde S$. We define the UMDP-Poly abstraction of System~\eqref{eq:sys} as $\U^\poly = (S,A,\Gamma^\poly)$, with 
    %
    \begin{multline}
        \label{eq:Gamma_poly}
        \Gamma_{s,a}^\poly := \{ \gamma \in \mathcal{P}(S) : \: \forall \tilde s \in \widetilde S_{s,a},\\
        \underline P(s,a,\tilde s) \le \sum_{s' \in \tilde s} \gamma(s') \le \overline P(s,a,\tilde s)
         \}
    \end{multline}
%
for all $s\in S_\safe$ and $a\in A$, where $\underline P(s,a,\tilde s)$ and $\overline P(s,a,\tilde s)$ are defined in~\eqref{eq:tp_bounds}, and $\Gamma_{s_\text{avoid}, a}^\poly := \{\delta_{s_\text{avoid}}\}$ for all $a \in A$.
%
\end{definition}


\begin{theorem}[Soundness of UMDP-Poly Abstraction]
\label{theorem:soundness}
    The UMDP $\U^\poly$ is a sound abstraction of System~\eqref{eq:sys}.
\end{theorem}
%
\begin{proof}
    First, fix $s\in S_\safe$, $a\in A$ and $x\in s$, and note that, since the regions in the partition $S$ are disjoint, it holds that $\sum_{s'\in \tilde s} \kernel(s' \mid x, a) = \kernel(\tilde s \mid x, a)$. Furthermore, by Lemma~\ref{lemma:tp_bounds}, this quantity belongs to the interval $[\underline P(s,a,\tilde s), \overline P(s,a,\tilde s)]$, implying that $\kernel(\cdot \mid x, a) \in \Gamma_{s,a}^\poly$.
\end{proof}

As mentioned above, $\Gamma^\poly$ represents uncertainty in the transitions more tightly than IMDPs and the $2$-layer abstractions with non-overlapping clusters proposed in \cite{gracia2024temporal}. This tighter $\Gamma^\poly$ results in higher-quality solutions at the expense of higher computation times, as we empirically show in \ig{(REF)}.

\begin{remark}
\label{rem:confidence}
    As pointed out in \cite{gracia2024temporal}, when $P_w$ is unknown, for a fixed number of samples $N$ and a fixed confidence of the abstraction being sound, the bounds in \eqref{eq:tp_bounds} become looser as the number of constraints
    in \eqref{eq:Gamma_poly} increases, i.e., $|\widetilde S|$. For this reason, imposing more constraints on the definition of $\Gamma^\poly$ would seem counterproductive in the data-driven setting. However, since this dependence is small (at most $\mathcal{O}(\log(|\widetilde S|)^{0.5})$), in practice polytopic UMDPs yield better results than both IMDPs and the UMDPs in \cite{gracia2024temporal}, even when $P_w$ is unknown.
\end{remark}

In order to fully deal with the issue mentioned in Remark~\ref{rem:confidence} and to speed up computations, we present a second abstraction class below.

\subsection{UMDP-ST Abstraction}
\label{sec:MDP_IST_abstraction}

The computation of the ambiguity set $\Gamma^\poly$ in Definition~\ref{def:mdp_poly_abstraction} can be expensive, as the bounds in~\eqref{eq:tp_bounds} need to be generated for all $(s,a,c,\tilde s)$ tuples. To mitigate this while avoiding significant conservatism, 
given $(s,a,c)$,
it is desirable to design the clusters $\tilde s \in \widetilde S_{s,a}$ in a way that minimizes $|\widetilde S|$
% given a $(s,a,c)$ tuple, one would like to design the clusters $\tilde s \in \widetilde S_{s,a}$ in such a way that $|\widetilde S|$ is as small as possible 
(see also Remark~\ref{rem:confidence}), 
while still retaining the essential information about the dynamics of System~\eqref{eq:sys}.
% while still encoding the relevant information about the dynamics of System~\eqref{eq:sys}. 
% We propose defining $\widetilde S$ in such a way that for each $c\in C$ there is a $q_{s,a,c} \in \widetilde S_{s,a}$ which contains only the states $s' \in S_{s,a}$ with $\mathrm{Reach}(s,a,c) \cap s' \neq\emptyset$. % In this case, Expressions~\eqref{eq:tp_bounds_lower} and \eqref{eq:tp_bounds_upper} collapse to the same quantity.
To this end, we propose defining the sets $\widetilde S_{s,a}$ such that for each $c \in C$, there exists a $q_{s,a,c} \in \widetilde S_{s,a}$ that includes only the states $s' \in S_{s,a}$ for which $\mathrm{Reach}(s,a,c) \cap s' \neq \emptyset$.

% When the probability distribution $P_w$ is known, the resulting polytopic UMDP abstraction becomes an MDP with Set-valued Transition probabilities (MDP-ST)~\cite{trevizan2007planning}, a special case of UMDP.  In these models, the successor state of a given $(s,a)$ belongs to the cluster $q_{s,a,c}$ with probability $P_w(c)$, and then, the adversary chooses the successor state from $s' \in q_{s,a,c}$ in a non-deterministic way.

When the probability distribution $P_w$ is known, the resulting polytopic UMDP abstraction becomes an MDP with Set-valued Transition probabilities (MDP-ST)~\cite{trevizan2007planning}, which is a special case of UMDPs. In these models, the successor state of a given $(s,a)$ pair belongs to the cluster $q_{s,a,c}$ with probability $P_w(c)$, and then the adversary non-deterministically selects the successor state $s'$ from $q_{s,a,c}$.

Nevertheless, in the case that $P_w$ is unknown, we must first learn the probabilities $P_w(c)$ from data, which results in a more complex abstraction, which we call Uncertain MDP-ST (UMDP-ST). In Proposition~\ref{prop:learning_P}, we leverage a multilayer partition of $C$ to learn $P_w$ as a polytopic set.

% Note that in this setting, one needs to estimate the bounds in \eqref{eq:tp_bounds} from data, and it is

%relies on checking wether or not $\mathrm{Reach}(s,a,c)$ is fully contained in $\tilde s$ per Expression~\eqref{eq:tp_bounds_lower}. 

\begin{proposition}[Learning $P_w$]
\label{prop:learning_P}
Let $C$ be a partition of $W$, and $\widetilde C$ be a set of clusters $\tilde c$ of the regions in $C$. Define $P_{w,C}\in \mathcal{P}(C)$ by discretizing $P_w$ according to $C$, i.e., $P_{w,C}(c) := P_w(c)$ for all $c \in C$. Given $N$ samples from $P_w$ and a confidence level $\alpha \in (0, 1)$, there exist explicit functions $\underline P_{w,C}, \overline P_{w,C} : \widetilde C \rightarrow [0, 1]$ that depend on $N, \alpha$, such that $P_{w,C}$ belongs to the set
%
\begin{align}
\label{eq:Gamma_C}
    \Gamma_C := \{ \gamma \in \mathcal{P}(C) : \underline P_{w,C}(\tilde c) \le \sum_{c \in \tilde c} \gamma(c) \le \overline P_{w,C}(\tilde c) \}.
\end{align}
%
with confidence $1 - \alpha$.
    
\end{proposition}
%
In the interest of space, we omit the proof of Proposition~\ref{prop:learning_P}, which follows the same reasoning as that of \cite[Theorem 4.6]{gracia2024temporal}. As previously mentioned, when $P_w$ is known, $P_{w,C}$ can be obtained exactly, instead of bounding it with high confidence, by computing the measure of every set $c\in C$. Therefore, we let $\Gamma_C = \{P_{w,C}\}$, which is not subject to any confidence.


Next, we formalize our UMDP-ST abstraction and prove its soundness:

\begin{definition}[UMDP-ST Abstraction]
    \label{def:mdp_ist_abstraction}
    For all $s\in S_\safe$ and $a\in A$, define $q_{s,a,c} := \{s'\in S: s'\cap \mathrm{Reach}(s,a,c) \neq \emptyset\}$ for all $c\in C$, and let $Q_{s,a} := \{q_{s,a,c} : c \in C\}$. We define the UMDP-ST abstraction of System~\eqref{eq:sys} as $\U^\ST = (S,A,\Gamma^\ST)$, 
    with 
    % $\Gamma_{s,a}^\ST$ being the set of all $\gamma \in \mathcal{P}(S)$ that can be expressed as 
    %
    \begin{multline}
    \label{eq:feasible_distribution_mdp_ust}
    % \begin{split}
    \Gamma_{s,a}^\ST := \bigcup_{\substack{\gamma_C \in \Gamma_C\\ \alpha_q \in \mathcal{P}(q), \: \forall q\in Q_{s,a}}}\{ \gamma \in \mathcal{P}(S) : \forall s' \in S, \\
        \gamma(s') = \!\!\!\!\! \sum_{c \in C: s'\in q_{s,a,c}} \!\!\!\!\! \alpha_{q_{s,a,c}}(s') \gamma_C(c)\}.
        % \gamma(s') = \!\!\! \sum_{c \in C: s'\in q_{s,a,c}} \!\!\! \alpha_{q_{s,a,c}}(s') \gamma_C(c) \quad \text{for all}\:s' \in S,
        % \end{split}
    \end{multline}
%
We also define $\Gamma_{s_\unsafe,a}^\ST = \{\delta_{s_\unsafe}\}$ for all $a\in A$.
%
\end{definition}

\begin{remark}[IMDP-ST Abstraction]
    In the case that the set $\widetilde C$ in Proposition~\ref{prop:learning_P} contains all and only the singletons $\{c\}$ for all $c\in C$, it is evident that the constraints in~\eqref{eq:Gamma_C} become decoupled intervals across all $s'\in S$. This structure is the same as that of the set of transition probability distributions of an IMDP, and for this reason we denote the resulting abstraction an IMP-ST. In Section~\ref{sec:synthesis} we show how to leverage the structure of this abstraction class to design an efficient strategy synthesis algorithm.
\end{remark}


\begin{theorem}[Soundness of UMDP-ST Abstraction]
\label{theorem:soundness_umdp_ist}
    The UMDP-ST $\U^\ST$ is a sound abstraction of System~\eqref{eq:sys}.
\end{theorem}
%
\begin{proof}
    First, fix $s\in S_\safe$, $a\in A$ and $x\in s$. By the law of total probability we obtain that, for all $s'\in S$, $\kernel(s' \mid x, a) = \sum_{c\in C} P_w(\{w \in c : f(x,a,w) \in s'\})$. Note that if $s' \notin q_{s,a,c}$ or, equivalently, since $\mathrm{Reach}(x,a,c) \cap s' = \emptyset$, then $f(x,a,w) \notin s'$ for each $w \in c$, and thus $P_w(\{w \in c : f(x,a,w) \in s'\}) = 0$. Therefore, by conditioning on the event $\{w \in c\}$, we obtain $\sum_{c\in C} P_w(\{w \in c : f(x,a,w) \in s'\}) P_{w,C}(c) = \sum_{c\in C : s' \in q_{s,a,c}} P_w(\{w \in c : f(x,a,w) \in s'\}) P_{w,C}(c)$. Let $\alpha_{q_{s,a,c}}(s') := P_w(\{w \in c : f(x,a,w) \in s'\})/P_w(c)$, for all $s' \in S$. $c \in C$. Note that, for a given $c \in C$, $\alpha_{q_{s,a,c}} \in \mathcal{P}(q_{s,a,c})$, since it takes values in $[0, 1]$ and $\sum_{s'\in q_{s,a,c}} \alpha_{q_{s,a,c}}(s') = P(\cup_{s'\in q_{s,a,c}}\{ w \in c : f(x,a,w) \in s' \})/P_w(c) = P_w(\{ w \in c : f(x,a,w) \in \cup_{s'\in q_{s,a,c}} s' \})$. The last chain of equalities holds due to the regions in $S$ being disjoint, $f$ being a function and by definition of $q_{s,a,c}$. Therefore, for each $x\in s$, $\kernel(s' \mid x, a)$ is of the form in \eqref{theorem:soundness_umdp_ist}, with $\gamma_C = P_{w,C}$ which concludes the proof.
\end{proof}
%


\section{Controller Synthesis}
\label{sec:synthesis}

% In this section, we show how to compute strategies that maximize the reach-avoid probability, while being robust agianst all uncertainties embedded into the abstraction. Specifically, we describe how to perform synthesis for a general rectangular UMDP via unbounded-horizon robust dynamic programming, boiling down to solving linear optimization problems for both polytopic UMDPs and UMDP-STs 

In this section, we present a method for computing strategies that maximize the reach-avoid probability while remaining robust against all uncertainties embedded in the abstraction. Specifically, (i) we describe how to synthesize strategies for a general rectangular UMDP using unbounded-horizon Robust Dynamic Programming (RDP), and thus applying to polytopic UMDPs, UMDP-STs and IMDP-STs, (ii) we show that for these models RDP reduces to solving linear optimization problems
at each iteration, and (iii) we devise a tailored algorithm to efficiently solve these linear programs in the case of an IMDP-ST.

Given a UMDP $\U$, a strategy $\sigma\in \Sigma$, an adversary $\xi\in\Xi$ and an initial state $s_0\in S$, we denote the reach-avoid probability of $\U$ by $\text{Pr}_{s}^{\strategy,\xi}(\varphi)$, whose formal definition is analogous to \eqref{eq: satisfaction_prob}. 

%
\begin{proposition}[RDP {\cite[Theorem 6.2]{gracia2025efficient}}]
\label{prop:robust_value_iteration}
Given a rectangular UMDP $\U = (S,A,\Gamma)$, a reach-avoid specification $\varphi = (\Sreach, \{s_\text{avoid}\})$, and $s \in S$, define the optimal pessimistic (robust) unbounded-horizon reachability probability as 
%
\begin{align}
\label{eq:max_reachability_probability}
\underline p(s) :=\sup_{\sigma \in\Sigma}\inf_{\xi\in\Xi} \text{Pr}_{s}^{\strategy,\xi}(\varphi).
%
\end{align}
%
Consider also the recursion
%
\begin{align}
\label{eq:robust_value_iteration_lower_bound}
    \underline p^{k+1}(s) = 
        \begin{cases}
             1 &\text{if }\:s \in \Sreach\\
             0 &\text{if }\:s = s_\text{avoid}\\
             % s \in S\setminus S_\safe\\ 
             \max\limits_{a\in 
             A}\min\limits_{\gamma\in\Gamma_{s,a}} \sum\limits_{s\in 
             S}\gamma(s)\underline p^{k}(s) &\text{otherwise},
             \end{cases}
\end{align}
%
for all $k\in\uint$, with initial condition $\underline p^{0}(s) = 1$ for all $s\in \Sreach$ and $0$ otherwise. Then, recursion \eqref{eq:robust_value_iteration_lower_bound} converges to $\underline p$
.
\end{proposition}
%
Next, we obtain a stationary strategy $\sigma^*$ that achieves the supremum in~\eqref{eq:robust_value_iteration_lower_bound} as shown in \cite[Theorem 6.4]{gracia2025efficient}. 
Given this $\sigma^*$, we obtain the optimistic probability $\overline p(s) := \sup_{\xi\in\Xi} \text{Pr}_{s}^{\strategy^*,\xi}(\varphi)$ by iterating on the recursion in \cite[Equation 6.5]{gracia2025efficient}, which is similar to the one in \eqref{eq:robust_value_iteration_lower_bound} but where the $\min$ over $\Gamma_{s,a}$ is replaced by a $\max$, and where the actions are determined by $\sigma^*$. 

Given $\sigma^*$ on a sound UMDP abstraction, we map it to the controller $\kappa$ of System~\eqref{eq:sys} as $\kappa(\omegapathx) := \sigma^*(\omegapath)$ for all $\omegapathx \in \Omegapathxfin$, where $\omegapath$ is the equivalent path of $\omegapathx$ on $\U$. The following result establishes the satisfaction guarantees of System~\eqref{eq:sys} in closed loop with $\controller$:
%
\begin{theorem}[Correctness of the Controller]
\label{thm:strategy_synthesis}
    Let $\underline p$ be obtained via Proposition~\ref{prop:robust_value_iteration}, and $\sigma^*$, $\overline p$ and $\kappa$ be as explained afterwards. 
    %Furthermore, let $\controller$ be the controller obtained by refining $\sigma^*$ to System~\eqref{eq:sys}. 
    Then, for all $x_0\in \reals^n$, it holds that $\text{Pr}_{x_0}^{\controller}(\varphi) \in [\underline p(s), \overline p(s)]$, with $s\in S$ such that $x_0 \in s$.
\end{theorem}

\subsection{Inner Optimization Problems}

We now show that, when the abstraction is a polytopic UMDP or a UMDP-ST, the inner problems in recursion \eqref{eq:robust_value_iteration_lower_bound}, to be solved during RDP, are equivalent to linear programs.
%
\begin{theorem}[Inner Minimization for Polytopic UMDPs]
\label{th:RVI_LP}
Consider the RDP in \eqref{eq:robust_value_iteration_lower_bound} for the polytopic UMDP $\mathcal{U} = (S,A,\Gamma^\poly)$. Then, for every $k\in \uint$, $s\in S_\safe,$ and $a\in A$, the inner minimization problem in \eqref{eq:robust_value_iteration_lower_bound} is equivalent to the following linear program: 
\begin{align}
\label{eq:LP_cost}
\min_{\gamma} \;
\sum_{s'\in S}\gamma_{s'}\underline p^{k}(s'), \hspace{12em}
\end{align}\vspace{-1em}
%
\begin{subequations} \label{eq:feasible set_robust_MDP_cost} 
\begin{align}
{\rm s.t.} \;  \underline P(s,a,\tilde s) &\le \sum_{s'\in \tilde s} \gamma_{s'} \quad  &\forall \tilde s\in \widetilde S_{s,a}  \label{constraint:a} \\
\sum_{s'\in \tilde s} \gamma_{s'} &\le \overline P(s,a,\tilde s) \quad  &\forall \tilde s\in \widetilde S_{s,a} \label{constraint:b} \\
 \gamma_{s'} &\geq 0, &\forall s'\in S \label{constraint:c} \\
 \sum_{s'\in S} \gamma_{s'} &\ge 1& \label{constraint:d}
\end{align}
\end{subequations}
%
where $\underline P$ and $\overline P$ are defined in \eqref{eq:tp_bounds}.
\end{theorem}
%
\begin{proof}
    The proof is immediate by noting that $\Gamma_{s,a}^\poly$ is equivalent to the feasible set of \eqref{eq:Gamma_poly}.
\end{proof}

\iffalse

\begin{theorem}[Dual Reformulation of Problem~\ref{th:RVI_LP}]
\label{th:RVI_dual}
Problem \ref{th:RVI_dual} has the following dual: 
\begin{align}
\label{eq:dual_cost}
\min_{\lambda \ge 0, \upsilon \ge 0} \;
\sum_{q'\in Q_{s,a}} \big( \lambda(q')\underline P(s,a,q') - \upsilon(q')\overline P(s,a,q') \big)
\end{align}\vspace{-1em}
\begin{subequations} \label{eq:feasible set_dual} 
\begin{align}
{\rm s.t.} \;
\underline p^k(s') + \sum_{q'\ni s'} \big( \upsilon(q') - \lambda(q') \big) \ge 0 \quad \forall s' \in S.
\end{align}
\end{subequations}
\end{theorem}

\begin{theorem}[Convex Optimization Problem]
\label{th:RVI_convex}
Problem \ref{th:RVI_dual} has the following dual: 
\begin{align}
\label{eq:dual_cost}
\min_{\lambda \ge 0} \;
\sum_{q'\in Q_{s,a}} \lambda(q')\underline P(s,a,q') + \sum_{s'\in S} \overline P(s,a,s') \cdot \min\big\{\underline p^k(s') - \sum_{q'\ni s'} \lambda(q'), 0\big\}.
\end{align}
\end{theorem}

\fi


\begin{theorem}[Inner Minimization for UMDP-STs]
\label{th:RVI_mdp_ust}
Consider the RDP in~\eqref{eq:robust_value_iteration_lower_bound} for the UMDP-ST $\U^\ST = (S,A, \Gamma^\ST)$. Then, for every $k\in \uint$, $s\in S_\safe$ and $a\in A$, the inner minimization problem in \eqref{eq:robust_value_iteration_lower_bound} is equivalent to: 
%
\begin{align}
\label{eq:mdp_ust_cost}
&\min_{\gamma\in \Gamma_C} \;
\sum_{q'\in Q_{s,a}}\gamma(q')\underline p^{k}(q')
\end{align}%\vspace{-1em}
%
where $\underline p^{k}(q') = \min\{\underline p^{k}(s') : s' \in q'\}$ for all $q'\in Q_{s,a}$, and $\Gamma_C$ is of the form~\eqref{eq:Gamma_C}. Having computed $\underline p^{k}(q')$, optimization~\eqref{eq:mdp_ust_cost} becomes a linear program.
\end{theorem}
%
\begin{proof}
    Let $s\in S_\safe$ and $a\in A$. Note that, by the structure of $\Gamma_{s,a}$ in \eqref{eq:feasible_distribution_mdp_ust}, the inner problem in \eqref{eq:robust_value_iteration_lower_bound} is equivalent to
    %
    \begin{align*}
    \min_{\widetilde\gamma\in \Gamma_C} \min_{\{\alpha_{q_{s,a,c}} \in \mathcal{P}(q_{s,a,c})\}} \sum_{c \in C} \sum_{s' \in S\cap q_{s,a,c}} \alpha_{q_{s,a,c}}(s') \tilde\gamma_C(c)  \underline p^{k}(s').
\end{align*}
%
For each $\widetilde\gamma\in \Gamma_C$, the second $\min$ is a linear program, since the objective is linear in $\{\alpha_{q_{s,a,c}}\}$ and $\mathcal{P}(q_{s,a,c})$ is a polytope. As such, the optimal value is attained when each $\alpha_{q_{s,a,c}}$ is at a vertex of $\mathcal{P}(q_{s,a,c})$. Such an $\alpha_{q_{s,a,c}}$ assigns probability $1$ to a single state in $q_{s,a,c}$, and zero to all other states. Since each $\alpha_{q_{s,a,c}}$ is decoupled from the others, the minimum is attained when, for each $q_{s,a,c} \in Q_{s,a}$, $\alpha_{q_{s,a,c}}(s^*) = 1$ for some $s^*\in \arg\min\{\underline p^k(s') : s' \in q_{s,a,c}\}$, and $0$ otherwise. This yields
%
\begin{align*}
    \sum_{c\in C}\tilde\gamma_C(c)\min\{\underline p^k(s') : s' \in q_{s,a,c}\},
\end{align*}
%
which holds for all $\tilde\gamma_C \in \Gamma_C$, thus concluding the proof.
\end{proof}

Theorems~\ref{th:RVI_LP} and \ref{th:RVI_mdp_ust} show that standard linear programming solvers can be employed to solve the inner problems in \eqref{eq:robust_value_iteration_lower_bound} during value iteration. In addition to this, in the case of UMDP-STs, the maximum $\underline p^k(s')$ on each $q_{s,a,c}$ needs to be found, which adds negligible computational burden.


\begin{remark}[Inner Minimization for IMDP-STs]
    In the case of UMDP-STs, if the set $\Gamma_C$ is defined by intervals, this is, when the clusters $\tilde c \in C$ in its definition \eqref{eq:Gamma_C} are non-overlapping singletons, the optimization problem in~\eqref{eq:mdp_ust_cost} is the same as the inner problems found in IMDPs, and can hence be efficiently solved using the well-known O-maximization algorithm \cite{givan2000bounded}. (\ig{MAYBE THM? HOW TO WORD IT?})
\end{remark}


\section{More Stuff...}

\begin{lemma}
\label{lemma:imdp_vs_mdpst}
    Let $C$ be a partition of $W$, $P_w$ be known and $S, A$ be obtained as in... Denote by $\Gamma^\text{IMDP}$ and $\Gamma^\text{ST}$ the sets of transition probability distributions of the IMDP and MDP-ST abstractions as defined in... Then, $\Gamma_{s,a}^\text{IMDP} \subseteq \Gamma_{s,a}^\text{ST}$.
\end{lemma}
%
\begin{proof}
    Given $\gamma \in \Gamma_{s,a}^\text{IMDP}$, we prove that $\gamma \in \Gamma_{s,a}^\text{ST}$. Note that $\gamma \in \Gamma_{s,a}^\text{IMDP}$ implies existence of distributions $\{\alpha_{q_{s,a,c}}\}_{c\in C} \subset \mathcal{P}(q_{s,a,c})$ such that $\gamma(s') = \sum_{c \in C}\mathds{1}_{q_{s,a,c}}(s')\alpha_{q_{s,a,c}}(s')P_w(c)$ for all $s'\in S$. Given $s'\in S$, we first prove that $\underline P(s,a,s') \le \gamma(s')$ by proving that the sufficient condition $\boldsymbol{1}( \mathrm{Reach}(s,a,c) \subseteq s' ) \le \mathds{1}_{q_{s,a,c}}(s')\alpha_{q_{s,a,c}}(s')$ for all $c \in C$ holds. Fix $c \in C$ and, note that, if $\mathrm{Reach}(s,a,c) \subseteq s'$, then $\mathrm{Reach}(s,a,c) \cap s'' = \emptyset$ for all $s''\in S\setminus \{s'\}$, and therefore it holds that $q_{s,a,c} = \{s'\}$, $\alpha_{q_{s,a,c}} = \delta_{s'}$, and $\mathds{1}_{q_{s,a,c}}(s')\alpha_{q_{s,a,c}}(s') = \boldsymbol{1}( \mathrm{Reach}(s,a,c) \subseteq s' ) = 1$. On the other hand, if $\mathrm{Reach}(s,a,c) \not\subseteq c$, then $\mathds{1}_{q_{s,a,c}}(s')\alpha_{q_{s,a,c}}(s') \ge \boldsymbol{1}( \mathrm{Reach}(s,a,c) \subseteq s' ) = 0$. Since this holds for all $c\in C$, it follows that $\underline P(s,a,s') \le \gamma(s')$. Next, we follow the previous logic to prove that $\overline P(s,a,s') \ge \gamma(s')$. Fix $c\in C$ and note that $\mathrm{Reach}(s,a,c) \cap s' \neq \emptyset$ iff $s'\in q_{s,a,c}$. Therefore, $\mathds{1}_{q_{s,a,c}}(s')\alpha_{q_{s,a,c}}(s') \le \boldsymbol{1}( \mathrm{Reach}(s,a,c) \cap s' \neq \emptyset ) = 1$. Since this holds for all $c\in C$, we obtain $\overline P(s,a,s') \ge \gamma(s')$. Furthermore, since the previous bounds on $\gamma(s')$ hold for all $s'\in S$, we obtain that $\gamma\in \Gamma_{s,a}^\text{IMDP}$, which concludes the proof.
\end{proof}

\begin{remark}
    The relation between $\Gamma_{s,a}^\text{IMDP}$ and $\Gamma_{s,a}^\text{ST}$ in Theorem~\ref{thm:imdp_vs_st} is not an equality in general. As a counterexample, consider a setting where $C = \{c_1, c_2\}$, $P(c_1) = P(c_2) = 1/2$, $q_{s,a,c_1} = \{s_1, s_2\}$ and $q_{s,a,c_2} = \{s_3, s_4\}$. From Expression \ig{(REF)}, the interval bounds that define $\Gamma_{s,a}^\text{IMDP}$ are $\underline P(s,a,s') = 0$ for all $s'\in S$ and $\overline P(s,a,s') = 1/2$ for all $s'\in\{s_1, s_2, s_3, s_4\}$ and $\overline P(s,a,s') = 0$ for all $s'\in S\setminus \{s_1, s_2, s_3, s_4\}$. Note that the distribution $\gamma^\text{IMDP} = 1/2(\delta_{s_1} + \delta_{s_2})$ belongs to $\Gamma_{s,a}^\text{IMDP}$ as it respects said interval bounds. Note also that any distribution in $\gamma_{s,a}^\text{ST}$ should be expressible as, for some distributions $\alpha_{q_{s,a,c_1}} \in \mathcal{P}(q_{s,a,c_1})$ and $\alpha_{q_{s,a,c_2}} \in \mathcal{P}(q_{s,a,c_2})$, $\gamma^\text{ST}(s') = \mathds{1}_{q_{s,a,c_1}}( s' )\alpha_{q_{s,a,c_1}}(s')P(c_1) + \mathds{1}_{q_{s,a,c_2}}( s' )\alpha_{q_{s,a,c_2}}(s')P(c_2)$ for all $s'\in S$. This implies that, regardless of the choice of $\alpha_{q_{s,a,c_1}}$ and $\alpha_{q_{s,a,c_2}}$, $\gamma^\text{ST}(s_3) + \gamma^\text{ST}(s_4) = \alpha_{q_{s,a,c_2}}(s_3)P(c_2) + \alpha_{q_{s,a,c_2}}(s_4)P(c_2) = P(c_2) = 1/2$, which clearly $\gamma^\text{IMDP}$ does not satisfy, as $\gamma^\text{IMDP}(s_3) + \gamma^\text{IMDP}(s_4) = 0$.
\end{remark}

\begin{theorem}
\label{thm:imdp_vs_imdpst}
    Let $C$ be a partition of $W$, $P_w$ be unknown and $S, A$ be obtained as in... Denote by $\Gamma^\text{IMDP}$ and $\Gamma^\text{IST}$ the sets of transition probability distributions of the IMDP and IMDP-ST abstractions as defined in..., for the same confidence $1-\alpha$. Then, $\Gamma_{s,a}^\text{IMDP} \subseteq \Gamma_{s,a}^\text{IST}$.
\end{theorem}
%
\begin{proof}
    
\end{proof}

\iffalse

\subsection{Heuristics for the Inner Minimization Problem \eqref{eq:LP_cost} - \eqref{eq:feasible set_robust_MDP_cost}}

\subsubsection{Early Identification of non-Optimal actions}

\subsubsection{Warm-Starting of LPs}



\begin{algorithm}%[t]\small
 \caption{Inner minimization}\label{alg:inner_min}
 %\vspace{-4mm}
\begin{algorithmic}[1]
    \REQUIRE $\U, s\in S\setminus\{s_{|S|}\}, \underline p^k$, $\{\gamma_{s,a}^{k-1} : a \in A\}$
    \ENSURE $\underline p^{k+1}(s), \{\gamma_{s,a}^k : a \in A\}$
    \FOR{$a\in A$}
    \STATE $\lambda \gets \sum_{s' \in S} \gamma_{s,a}^{k-1}(s') \underline p^k(s') - \underline p^k(s)$
        \IF{$\lambda < 0$ // Action a is not optimal}
        \STATE $\widetilde{V}(s,a) \gets 0$
        \STATE $\gamma_{s,a}^k \gets \gamma_{s,a}^{k-1}$
        \ELSIF{$\gamma_{s,a}^{k-1}$ also attains $\min$ at iteration $k$}
        \STATE $\widetilde{V}(s,a) \gets \sum_{s' \in S} \gamma_{s,a}^{k-1}(s') \underline p^k(s')$
        \STATE $\gamma_{s,a}^k \gets \gamma_{s,a}^{k-1}$
        \ELSE
        \STATE $(\widetilde V(s, a), \gamma_{s,a}^k) \gets$ Solve LP \eqref{eq:LP_cost} - \eqref{eq:feasible set_robust_MDP_cost} initialize at $\gamma_{s,a}^{k-1}$ 
        \ENDIF
    \ENDFOR
    \STATE $\underline p^k(s) \gets \max\{\widetilde V(s, a) : a \in A\}$
\end{algorithmic}
\end{algorithm}

\fi



==> sections_old/case_studies_old.tex <==
\section{Case Studies}
\label{sec:case_studies}

In this section we empirically showcase the effectiveness of our approach to efficiently obtain UMDP abstractions and to synthesize controllers with tight satisfaction guarantees. We evaluate our results through two case studies: a 2D unicycle model and a nonlinear 3D Dubin's car model where the disturbance is nonlinear, and represents \emph{Coulomb friction}, which depends on the heading angle of the car, and noise in the yaw rate. The dynamics and exact setting of the case studies can be found in \cite{gracia2024temporal}.

Figure~\ref{fig:graphs} shows how both poly-UMDPs and UMDP-ST yield better results than IMDPs, which can be observed in a smaller $e_\text{avg}$. Furthermore, as the IMDP abstraction is refined, $e_\text{avg}$ grows instead of providing better results, and this is the case even for a 2-dimensional system and a relatively small partition of $40\times 40$ states. 

In the case of a polytopic UMDP abstraction, $e_\text{avg}$ also seems to slightly increase after the  On the other hand, in the case of poly-UMDPs, $e_\text{avg}$ seems to remain fairly constant, whereas for UMDP-STs it slowly decreases. When it comes to computation times, obtaining a UMDP-ST abstraction seems way less expensive than IMDP or poly-UMDPs, since the number of bounds of the form \eqref{eq:tp_bounds} to be computed is way lower, which was one of the motivations for exploring these abstraction (see Section~\ref{sec:MDP_IST_abstraction}). The time required to synthesize a controller is also smaller in UMDP-STs than in polytopic-UMDPs, as the set $\Gamma^\ST$ represents uncertainty more efficiently, i.e., involving less constraints, than $\Gamma^\poly$, while yielding a similar $e_\text{avg}$.

We remark that for the IMDP approach to provide non-vacuous results, we first learned a high-probability subset of the support of $P_w$, and then embedded that constraint into the set $\Gamma$ of the IMDP (see \cite{gracia2024temporal}). If we had not do this, the IMDP would yield vacuous satisfaction guarantees.

Additionally, we note that all experiments were run in MATLAB, and that there exist implementations of value iteration for IMDPs that are orders of magnitudes faster. Investigating a


%
\begin{figure*}
    \centering
    \begin{subfigure}{.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/e_avg.eps}
        \caption{}
    \end{subfigure}
    ~
    \begin{subfigure}{.32\textwidth}
    \centering
        \includegraphics[width=\linewidth]{images/abs_time.eps}
        \caption{}
    \end{subfigure}
    ~
    \begin{subfigure}{.32\textwidth}
        \includegraphics[width=\linewidth]{images/syn_time.eps}
        \caption{}
    \end{subfigure}
    \caption{Results of the 2D unicycle case study as a function of the size of the discretization, for $N = 2000$ samples from $P_w$. For the case of the IMDP, the support of $P_w$ had to be learned.}
    \label{fig:graphs}
\end{figure*}
%






==> sections_old/intro_old.tex <==
\section{Introduction}
\label{sec:introduction}

% \IEEEPARstart{T}{he}  

Stochastic systems serve as fundamental models for uncertain dynamical control systems, where ensuring \emph{probabilistic safety guarantees} is crucial for \emph{safety-critical} applications. However, providing such guarantees is challenging, especially for stochastic systems with general dynamics. A powerful approach to addressing this challenge is \textit{abstraction-based} synthesis, where a continuous-space stochastic system is represented by a finite-state Markov process with accurate modeling of the error bounds.
While existing abstraction methods have been successful in specific settings, they are often limited to particular classes of dynamics and suffer from the state-explosion problem, compromising both scalability and accuracy. This work aims to develop a general abstraction framework for discrete-time stochastic systems that improves accuracy while maintaining computational tractability, enabling more precise safety probability bounds.



A popular approach to verification and synthesis for continuous-space stochastic systems via finite abstraction.  

The paper introduction...
See, for instance \cite{Pippo,Pluto}.

Motivation...

Related works...

Abstraction-based approaches...

MDPs...

IMDPs...

UMDPs...

In this work we show how to obtain two different classes of UMDP abstractions, which leverage multi-layer partitions: polytopic UMDPs, in which the transition probability distributions are constrained to convex polytopes, and a variant of MDPs with set-valued transition probabilities, which we denote UMDP-STs.


MDPs with set-valued transition probabilities (MDP-STs) are first proposed in \cite{trevizan2007planning}, and have been recently explored in \cite{yu2025planning} under temporal logic specifications.

When the dynamics of the system are nonlinear, \cite{skovbekk2023formal} obtains an IMDP abstraction by partitioning the space of the disturbance and leveraging forward reachability.

Data-driven setting...

In the case that the dynamics are nonlinear and the probability distribution of the disturbances is unknown, \cite{gracia2024temporal} shows how a na\"ive use of IMDP abstractions results in an overly conservative abstraction which fails to provide meaningful results. This issue arises when the number of states in the abstraction is high, hence limiting the applicability of these methods in higher dimensions. Furthermore, refining the state-space partition, which intuitively should produce tighter results, even worsens this issue.


For this reason, that work proposes to employ UMDP abstractions instead, which encode more information about the dynamics of the original system, thus resulting in a tighter abstraction and better results. While the UMDPs proposed by \cite{gracia2024temporal} represent transition probability distributions as polytopes, \cite{gracia2024data} employs \emph{Wasserstein ambiguity sets}.



leverages on forward reachability computations and samples from the system to obtain a correct UMDP abstraction that

\cite{skovbekk2023formal} proposed a modified value iteration algorithm that leveraged reasoning about the probability of transitioning to clusters of states. Additionally, \cite{gracia2024temporal} considers a $2$-layer partition composed by a fine one and a coarse one, consisting of non-overlapping clusters of fine regions. Contrary to \cite{skovbekk2023formal}, \cite{gracia2024temporal} encodes this information into the abstraction, effectively separating this step from the synthesis one. We build on the method of \cite{gracia2024temporal}, and increase the tightness of the results by allowing disjoint clusters and multilayer partitions.

Contributions...

\begin{itemize}
    \item A novel framework to formal control of discrete-time stochastic systems under disturbances with a possibly uncertain distribution and (unbounded) reach-avoid specifications
    \item We propose two UMDP abstraction models that leverage a layered partition of the state (and disturbance) space. Specifically, our work is the first to consider an abstraction with set-valued transition probabilities
    \item An approach that effectively deals with the issues related to IMDP abstractions pointed out in \cite{gracia2024temporal}, and which yields improved results with respect to state-of-the-art
    \item Empirical evaluations through \ig{COMPLETE}
\end{itemize}

==> sections_old/preliminaries_old.tex <==
\section{Preliminaries: UMDP Semantics}
\label{sec:preliminaries}

% Since we assume a general nonlinear $f$, our abstractions rely on reachable set computations.
% %
% \begin{definition}[\text{Reach}]
%     The $1$-step forward reachable set of $s\subset \reals^n$, $u \in U$ and $c \in W$, is defined as $\text{Reach}(s,a,c) := \{f(x,a,w) : x\in s, w \in c\}$.
% \end{definition}
% %
% There exist numerous approaches to obtain overapproximations of forward reachable sets such as \ig{(CITE)}. We highlight that employing an overapproximation instead of the actual reachable set does not compromise the soundness of our framework, but only increases its conservatism.



% Given UMDP $\U$, 
% starting from state $s\in S$, the 
% let $s_0,\ldots,s_T \in S$, $a_0,\dots,a_{T-1}\in A$ and $T \in \mathbb{Z}_+$, such that there exists $\gamma\in\Gamma_{s_t,a_t}$ with $ \gamma(s_{t+1})> 0$ for all $k \in \{0, \dots, T-1\}$. We denote by $\omegapath =s_0 \xrightarrow{a_0}% x_1 \xrightarrow{u_1}  
% \ldots \xrightarrow{a_{T-1}} s_T$ a finite \emph{path} of length $|\omegapath| = T + 1$ of UMDP $\U$. 

For a given UMDP $\U$, we define a \textit{path} $\omegapath =s_0 \xrightarrow{a_0}
\ldots \xrightarrow{a_{T-1}} s_T$ to be a sequence of states such that for all $0 \leq t \leq T$, $s_t \in S$, and for all $0 \leq t \leq T-1$, $a_t \in A$ and there exists distribution $\gamma \in \Gamma_{s_t,a_t}$ with $\gamma(s_{i+1}) > 0$. 
%The length of $\omegapath$ denoted by $|\omegapath| = T$ is finite if $T < \infty$; otherwise, it is infinite. 
We let $\Omegapathfin$ and $\Omegapath$ be the sets of all paths of finite and infinite length, respectively.
% Given a path $\omegapath$, we denote its state at time $t$ by $\omegapath(t) = s_t$.

A \emph{strategy} of $\U$ is a function $\strategy: \Omegapathfin \rightarrow A$ that maps each finite path to the next action. We denote by $\Sigma$ the set of all strategies of $\U$. Given a finite path $\omegapath \in \Omegapathfin$ with last state $s_t$ and a strategy $\strategy \in \Sigma$, $\U$ transitions from $s_{t}$ under $a_t = \strategy(\omegapath)$ to $s_{t+1}$ according to some probability distribution in $\Gamma_{s_t,a_t}$, which is chosen by the adversary \cite{givan2000bounded}. Formally, an \emph{adversary} is a function $\adversary: S \times A \times \mathbb{Z}_+ \rightarrow \mathcal{P}(S)$ that maps each state $s_t$, action $a_t$, and time step $t$ to a transition probability distribution $\gamma\in\Gamma_{s_t,a_t}$, according to which $s_{t+1}$ is distributed. We let $\Adversary$ denote the set of all adversaries. 

Given an initial state $s_0\in S$, a strategy $\strategy\in\Setofpolicies$, and an adversary $\xi\in\Xi$, $\U$ collapses to a Markov chain, with a unique probability measure over its paths. With a slight abuse of notation, we also denote this measure by $\text{Pr}_{s_0}^{\strategy,\xi}$.



==> sections_old/problem_formulation_old.tex <==
\section{Problem Formulation}
\label{sec:problem_formulation}

We consider discrete-time stochastic systems of the form
%
\begin{align}
\label{eq:sys}
    \x_{t+1} = f_{u_t}(\x_t, u_t, \w_t),
\end{align}
%
where $\x_t \in \reals^n$ is the state of the system at time $t \in \uint$, 
% ($\uint$ denoting the nonnegative integers), 
$u_t \in U \subset \reals^m$ with $|U| < \infty$ is the control input\footnote{
While $U$ is finite, each of its elements may represent a continuous set of controllers (e.g., a partition of a continuous set), making this assumption non-restrictive.}, 
and $\w_t \in W \subseteq \reals^d$ is the disturbance (noise).
We assume $(\w_t)_{t \in \uint}$ is an \emph{i.i.d.} stochastic process where each $\w_t$ is a sample from some probability distribution $P_w$. 
This work considers two scenarios: (i) $P_w$ is \emph{known}, and (ii) $P_w$ is \emph{unknown} but $N$ i.i.d. samples 
%$(\w^i)_{i = 1}^N$ 
from it are available\footnote{Per \cite{gracia2024data}, in most systems the assumption of having access to noise samples can be relaxed to having access to state trajectory samples.}. 
% In the latter case, the results will hold with some confidence with respect to the choice of the samples. 
We let vector field $f:\reals^n \times U \times W \rightarrow \reals^n$ be (possibly) a nonlinear function of all its arguments, assuming only that it is Lipschitz continuous on the third argument, $\w_t$ (see \cite[Assumption 2.1]{gracia2024temporal} for a detailed statement).

\iffalse
The only assumption we impose on $f$ is that, for each $u\in U$, $f$ is Lipschitz continuous on $w$, with a uniform Lipschitz constant over $x$ in some set $X_\safe \subseteq \reals^n$ (see \cite[Assumption 2.1]{gracia2024temporal} for a formal statement).
\fi

Given $x_0,\ldots,x_T \in \mathbb{R}^n$, $u_0,\dots,u_{T-1}\in U$, and $T \in \mathbb{Z}_+$, we define a finite \textit{trajectory} of System~\eqref{eq:sys} as $\omegapathx =x_0 \xrightarrow{u_0}
% x_1 \xrightarrow{u_1}  
\ldots \xrightarrow{u_{T-1}} x_T$ with length $|\omegapathx| = T + 1$. 
We denote by $\Omegapathxfin$ and $\Omegapathx$ the sets of all trajectories of finite and infinite lengths, respectively. %and denote the last state of $\omegapathx \in \Omegapathfin$ by $\text{last}(\omegapathx)$. 
The state of a trajectory $\omegapathx$ at time $t$ is denoted by $\omegapathx(t)$. 

We define a \emph{controller} of System~\eqref{eq:sys} as a function $\kappa: \Omegapathxfin \to U$ that maps each finite trajectory $\omegapathx$ to a control $u \in U$. 
Given a state-control pair $(x_t,u_t)$ and a Borel set $B$, the (measurable) \emph{transition kernel} $\kernel:\mathcal{B}(\reals^n)\times \reals^n\times U \rightarrow [0, 1]$
of System~\eqref{eq:sys} determines the probability that $x_{t+1} \in B$, i.e.,
$\kernel(B\mid x,u) = \int_W \mathds{1}_{B}(f(x,u,w))P_w(dw)$, where 
$P_w(c)$ is the probability measure of $c \subseteq W$, and
$\mathds{1}_B(x) = 1$ if $x \in B$, and $0$ otherwise. Given a controller $\controller$ and an initial state $x_0\in\reals^n$, the kernel $\kernel$ defines a unique probability measure $\text{Pr}_{x_0}^{\controller}$ over the trajectories of System~\eqref{eq:sys}~\cite{bertsekas1996stochastic}. 
%In this way, $\text{Pr}_{x_0}^{\controller}[\omegapathxbold(t) \in B]$ denotes the probability that $\x_t$ belongs to the set $B\in \mathcal{B}(\reals^n)$ when following strategy $\controller_x$ from initial state $x_0$. \ig{We probably don't need this last sentence.}

% We are interested in computing a controller, under which System~\ref{eq:sys} achieves a complex temporal requirement defined over regions of interests in $\reals^n$ with a high probability. Such specifications are typically expressed using temporal logic (e.g., LTL and LTLf). It is well-known that such properties boil down to reach-avoid properties over an extension of $\reals^n$.  For simplicity of presentation, we focus on such properties.

We aim to compute a controller for System~\eqref{eq:sys} that satisfies a complex temporal requirement over regions in $\reals^n$ with high probability. These specifications, often expressed in temporal logic (e.g., LTL, LTLf), reduce to reach-avoid properties over an extended state space via a finite abstraction. For simplicity of presentation, we focus on these properties and accurate finite abstractions in this work.

% In this work, we are interested in reach-avoid specifications. 
Given the sets $\Xreach, \Xavoid \subseteq \reals^n$ with $\Xreach \subseteq (\reals^n\setminus \Xavoid) =: \Xsafe$, we denote by $\varphi \equiv (\Xreach, \Xavoid)$ a reach-avoid specification. The probability that System~\eqref{eq:sys} reaches $\Xreach$ while avoiding $\Xavoid$ under controller $\controller$ from an initial state $x_0 \in \reals^n$ is formally defined as
%
\begin{multline}
    \label{eq: satisfaction_prob}
    \text{Pr}_{x_0}^{\controller}(\varphi) = \text{Pr}_{x_0}^{\controller}\big(\big\{\omegapathxbold \in \Omegapathx \mid \exists t \in \mathbb{Z}_+ \text{ s.t. }   
     \omegapathxbold(t)\in\Xreach \\
     \land \; \forall \,t' \le t, \; \omegapathxbold(t')\notin \Xavoid \big\} \big),
\end{multline}
%
% for which we use the shorthand $\text{Pr}_{x_0}^{\controller}(\varphi)$. 
% While we limit ourselves to reach-avoid specifications for clarity, we highlight that these are the basic building block to more general specifications like the ones expressed as \emph{temporal logic} formulas \ig{(CITE)}.

% A popular approach to synthesize a controller for System~\eqref{eq:sys} that yields a high and guaranteed reach-avoid probability relies on obtaining a finite abstraction of the system in the form of a UMDP.

To obtain an abstraction for System~\eqref{eq:sys} for the purposes of controller synthesis, a $\varphi$-respecting partition is needed.
\begin{definition}[$\varphi$-respecting Partition]
    A finite partition $S = \{s_1, \ldots, s_{|S|-1}, s_\text{avoid}\}$ of $\reals^n$ is called $\varphi$-respecting 
    % for sets $\Xsafe, \Xreach, \Xavoid, \subseteq \reals^n$ 
    if (i)  $S_\safe := \cup_{i=1}^{|S|-1} s_i = \Xsafe$, (ii) $s_\text{avoid} = \Xavoid$, and (iii) there exists subset $S_\text{reach} \subseteq S_\safe$ s.t. $\cup_{s \in S_\text{reach}} s = \Xreach$.
\end{definition}


% \begin{definition}[UMDP]
%     An uncertain MDP (UMDP) is a tuple $\U = (S, A, \Gamma)$, where $S$ and $A$ are finite sets of states and actions, respectively, and $\Gamma \equiv \{\Gamma_{s,a} : s\in S, a \in A\}$, where $\Gamma_{s,a}$ is the set of \emph{transition probability distributions} corresponding to state-action pair $(s,a)$.
% \end{definition}

\begin{definition}[UMDP Abstraction]
    \label{def: UMDP abstraction}
    Given $\varphi$-respecting partition $S$, 
    an uncertain MDP (UMDP) abstraction for System~\eqref{eq:sys} is a tuple $\U = (S, A, \Gamma)$, where $A = U$, and $\Gamma = \{\Gamma_{s,a} : s\in S, a \in A\}$, where $\Gamma_{s,a}$ is the set of \emph{transition probability distributions} corresponding to the pair $(s,a)$.
\end{definition}

% The abstraction process leverages a finite partition $S_\safe$ of $X_\safe$ that respects $\Xreach$, i.e., for each $s\in S_\safe$, $s\cap \Xreach$ is either empty or equal to $s$. We define the set of safe states of the abstraction as $S_\safe$. Additionally, we also let $s_\text{unsafe} := \Xunsafe$ denote the unsafe set, and define $S := S_\safe\cup \{s_\text{unsafe}\}$. Note that $s$ denotes both a state of $\U$ and a region of $\reals^n$. Next, we define the set of actions $\U$ be $A := U$.

%
% \begin{definition}[Sound UMDP Abstraction]
%     Given System \eqref{eq:sys} and a safe set $X_\safe$, a UMDP abstraction $\U = (S, A, \Gamma)$ is denoted \emph{sound} if for every $s\in S_\safe$, $a\in A$ it holds that: (i) the distribution $\gamma_{x,a} \in \mathcal{P}(S)$, given by $\gamma_{x,a}(s') := \kernel(s' \mid x, a)$ for all $s'\in S$, is contained in $\Gamma_{s,a}$, and  (ii) $\Gamma_{s_\unsafe, a} = \{\delta_{s_\unsafe}\}$.
% \end{definition}
%

\begin{definition}[Sound UMDP Abstraction]
    \label{def:sound UMDP abstraction}
    A UMDP abstraction $\U = (S, A, \Gamma)$ in Def.~\ref{def: UMDP abstraction} is \emph{sound} if (i) for every $s\in S_\safe$, $x \in s$, $a\in A$, the distribution $\gamma_{x,a}:= \{\gamma_{x,a}(s') = \kernel(s' \mid x, a) \mid s'\in S\} \in \Gamma_{s,a}$, and  (ii) $\Gamma_{s_\text{avoid}, a} = \{\delta_{s_\text{avoid}}\}$, where $\delta_{s_\unsafe}$ being the Dirac measure on $s_\unsafe$.
\end{definition}

We now have all the ingredients to formalize the problem(s) that we consider in this work.
%
% \begin{problem}[UMDP Abstraction]
%     \label{prob:problem1}
%     Obtain a sound UMDP abstraction $\U$ of System~\eqref{eq:sys}.
% \end{problem}
% %
% In order to solve Problem~\ref{prob:problem1}, we propose two UMDP classes which leverage multilayer partitions of $\Xsafe$ and $W$ respectively. Once obtained such an abstraction, we employ it to synthesize a controller for System~\eqref{eq:sys}.
% %
% \begin{problem}[Controller Synthesis]
%     \label{prob:problem2}
%     Given System~\eqref{eq:sys}, a reach-avoid specification $\varphi = (\Xreach, \Xavoid)$ and the corresponding sound UMDP abstraction $\U$, obtain a controller $\kappa$ and high probability functions $\underline p, \overline p:\reals^n \rightarrow [0, 1]$ such that
%     %
%     %\begin{align}
%         $\rm{Pr}_{x_0}^{\kappa}(\varphi) \in [\underline p(x_0), \overline p(x_0)]$ for all $x_0\in\reals^n$.
%     %\end{align}
%     %
%     \end{problem}
% 
% In this work we follow an abstraction-based approach: we obtain a finite-state UMDP representation of System~\eqref{eq:sys} that captures all of its behaviors. Then, we synthesize a strategy for this abstraction, which (robustly) maximizes its probability of the satisfying $\varphi$, and which we later correctly refine to the original system while preserving the satisfaction guarantees.

\begin{problem}
    Given System~\eqref{eq:sys}, reach-avoid property $\varphi = (\Xreach, \Xavoid)$, and $\varphi$-respecting partition $S$,
    \begin{enumerate}
        \item[1.] construct a sound UMDP abstraction $\U$, and
        \label{prob:problem1}
        \item[2.] using $\U$, synthesize controller $\kappa$ and high probability functions $\underline p, \overline p:\reals^n \rightarrow [0, 1]$ such that
        $\rm{Pr}_{x_0}^{\kappa}(\varphi) \in [\underline p(x_0), \overline p(x_0)]$ for all $x_0\in\reals^n$.
        \label{prob:problem2}
    \end{enumerate}    
\end{problem}

% This problem is well-established in the literature and several abstraction methods already exist.  Our approach, however, is different in that our method of abstraction often admits a higher lower bound $\underline p(x_0)$ for $\rm{Pr}_{x_0}^{\kappa}$ and tighter error $\overline p(x_0) - \underline p(x_0)$ than existing methods for the the same partition $S$.  The advantage of method lies in constructing a better representation of the ambiguity set $\Gamma$ for the transition probabilities of $\U$ using multiple levels of discretizations.  

This problem is well-studied, and several abstraction methods already exist. Our approach, however, differs in that it often provides a higher lower bound $ \underline{p}(x_0) $ for $ \Pr_{x_0}^{\kappa} $ and a tighter error bound $ \overline{p}(x_0) - \underline{p}(x_0) $ than existing methods for the same partition $S$, without requiring refinement. The key advantage lies in constructing a more precise representation of the ambiguity set $ \Gamma $ for the transition probabilities of $ \mathcal{U} $ using multiple levels of discretization by merging elements of $S$.



